On the verification of Embeddings using Hybrid Markov Logic

The standard approach to verify representations learned by Deep Neural Networks is to use them in specific tasks such as classification or regression, and measure their performance based on accuracy in such tasks. However, in many cases, we would want to verify more complex properties of a learned representation. To do this, we propose a framework based on a probabilistic first-order language, namely, Hybrid Markov Logic Networks (HMLNs) where we specify properties over embeddings mixed with symbolic domain knowledge. We present an approach to learn parameters for the properties within this framework. Further, we develop a verification method to test embeddings in this framework by encoding this task as a Mixed Integer Linear Program for which we can leverage existing state-of-the-art solvers. We illustrate verification in Graph Neural Networks, Deep Knowledge Tracing and Intelligent Tutoring Systems to demonstrate the generality of our approach.

==> expts.tex <==
% \section{Experiments}

% Datasets used
% Node embedding generation using different approaches
% How to formulate the HMLN problem
% relationship between distance and class
% What results can we show?

% For our experiments, we use the Cora graph dataset. It consists of 2708 nodes and 10556 edges which represent the articles and citation relationship between them. One property that we verify for this dataset is- two articles that have a citation relationship and are closer to each other in the embedding space share the same class label. We formulate the HMLN formulas as follows:
% $
% Dist(x,y) < \tau * (Class(x) \longleftrightarrow Class(y))\\
% $

% \begin{tikzpicture}[baseline, trim axis left]
% \begin{axis}[
% 				xlabel={Epochs},
% 				ylabel={MAP Objective bounds},
% 				xmin=0, xmax=8,
% 				ymin=-30000, ymax=30000,
% 				legend pos=south east,
% 				ymajorgrids=true,
% 				grid style=dashed,
% 				legend style={nodes={scale=0.75, transform shape}}
% 		]

%         \addplot[color=red, mark=triangle, smooth]
%             table[x=epoch, y=diff_true] {gat-original.dat};
%         \addplot [name path=upper, draw=none, forget plot] table[x=epoch,y=true_max] {gat-original.dat};
%         \addplot [name path=lower, draw=none, forget plot] table[x=epoch,y=true_min] {gat-original.dat};
%         \addplot [fill=red!10, forget plot] fill between[of=upper and lower];
% 			\addlegendentry{GAT Original True}

%         \addplot[color=red, mark=o, smooth]
%             table[x=epoch, y=diff_false] {gat-original.dat};
%         \addplot [name path=upper, draw=none, forget plot] table[x=epoch,y=false_max] {gat-original.dat};
%         \addplot [name path=lower, draw=none, forget plot] table[x=epoch,y=false_min] {gat-original.dat};
%         \addplot [fill=red!10, forget plot] fill between[of=upper and lower];
% 			\addlegendentry{GAT Original False}

%         \addplot[color=blue, mark=triangle, smooth]
%             table[x=epoch, y=diff_true] {gat-noisy.dat};
%         \addplot [name path=upper, draw=none, forget plot] table[x=epoch,y=true_max] {gat-noisy.dat};
%         \addplot [name path=lower, draw=none, forget plot] table[x=epoch,y=true_min] {gat-noisy.dat};
%         \addplot [fill=blue!10, forget plot] fill between[of=upper and lower];
% 			\addlegendentry{GAT Noisy True}

%         \addplot[color=blue, mark=o, smooth]
%             table[x=epoch, y=diff_false] {gat-noisy.dat};
%         \addplot [name path=upper, draw=none, forget plot] table[x=epoch,y=false_max] {gat-noisy.dat};
%         \addplot [name path=lower, draw=none, forget plot] table[x=epoch,y=false_min] {gat-noisy.dat};
%         \addplot [fill=blue!10, forget plot] fill between[of=upper and lower];
% 			\addlegendentry{GAT Noisy False}

%     \end{axis}
% \end{tikzpicture}

% \begin{figure*}

%     % \centering
%     \subfigure[GraphSAGE CORA]{\scalebox{0.7}{
%         \begin{tikzpicture}%[baseline, trim axis left]
%             \begin{axis}[
%     				xlabel={Epochs},
%     				ylabel={Test Accuracy},
%     				xmin=0, xmax=100,
%     				ymin=0, ymax=1,
%     				legend pos=south east,
%     				ymajorgrids=true,
%     				grid style=dashed,
%     				legend style={nodes={scale=0.75, transform shape}}
%     		]
    
%                 \addplot[color=red, mark=triangle, smooth]
%                     table[x=Epoch, y=Spec] {graphsage-accuracy.dat};
%                     \addlegendentry{Original GraphSAGE}
                    
%                 \addplot[color=blue, mark=x, smooth]
%                     table[x=Epoch, y=Light] {graphsage-accuracy.dat};
%                     \addlegendentry{Light Noise GraphSAGE}
                    
%                 \addplot[color=orange, mark=o, smooth]
%                     table[x=Epoch, y=Extreme] {graphsage-accuracy.dat};
%                     \addlegendentry{Extreme Noise GraphSAGE}
%             \end{axis}
%         \end{tikzpicture}
%         \label{graphsage_cora_accuracy}
%         }
%     }
%     \subfigure[GCN CORA]{\scalebox{0.7}{
%         \begin{tikzpicture}%[baseline, trim axis left]
%             \begin{axis}[
%     				xlabel={Epochs},
%     				ylabel={Test Accuracy},
%     				xmin=0, xmax=100,
%     				ymin=0, ymax=1,
%     				legend pos=south east,
%     				ymajorgrids=true,
%     				grid style=dashed,
%     				legend style={nodes={scale=0.75, transform shape}}
%     		]
    
%                 \addplot[color=red, mark=triangle, smooth]
%                     table[x=Epoch, y=Spec] {gcn-accuracy.dat};
%                     \addlegendentry{Original GCN}
                    
%                 \addplot[color=blue, mark=x, smooth]
%                     table[x=Epoch, y=Light] {gcn-accuracy.dat};
%                     \addlegendentry{Light Noise GCN}
                    
%                 \addplot[color=orange, mark=o, smooth]
%                     table[x=Epoch, y=Extreme] {gcn-accuracy.dat};
%                     \addlegendentry{Extreme Noise GCN}
%             \end{axis}
%         \end{tikzpicture}
%         \label{gcn_cora_accuracy}
%         }
%     }
%     \subfigure[GAT CORA]{\scalebox{0.7}{
%         \begin{tikzpicture}%[baseline, trim axis left]
%             \begin{axis}[
%     				xlabel={Epochs},
%     				ylabel={Test Accuracy},
%     				xmin=0, xmax=100,
%     				ymin=0, ymax=1,
%     				legend pos=south east,
%     				ymajorgrids=true,
%     				grid style=dashed,
%     				legend style={nodes={scale=0.75, transform shape}}
%     		]
    
%                 \addplot[color=red, mark=triangle, smooth]
%                     table[x=Epoch, y=Spec] {gat-accuracy.dat};
%                     \addlegendentry{Original GAT}
                    
%                 \addplot[color=blue, mark=x, smooth]
%                     table[x=Epoch, y=Light] {gat-accuracy.dat};
%                     \addlegendentry{Light Noise GAT}
                    
%                 \addplot[color=orange, mark=o, smooth]
%                     table[x=Epoch, y=Extreme] {gat-accuracy.dat};
%                     \addlegendentry{Extreme Noise GAT}
%             \end{axis}
%         \end{tikzpicture}
%         \label{gat_cora_accuracy}
%         }
%         \caption{Illustrating the Test Accuracy performance of GraphSAGE, GCN and GAT on the Cora graph dataset}
%     }
    
% \end{figure*}

% \begin{figure*}

%     \centering
%     \subfigure[Light Ep0]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/light_0.png}
%         \label{light_ep0}
%         }
%     }
%     \subfigure[Light Ep1]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/light_1.png}
%         \label{light_ep1}
%         }
%     }
%     \subfigure[Light Ep2]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/light_2.png}
%         \label{light_ep2}
%         }
%     }
%     \subfigure[Light Ep3]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/light_3.png}
%         \label{light_ep3}
%         }
%     }
%     \subfigure[Light Ep4]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/light_4.png}
%         \label{light_ep4}
%         }
%     }
%     \subfigure[Light Ep5]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/light_5.png}
%         \label{light_ep5}
%         }
%     }
%     \subfigure[Light Ep6]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/light_6.png}
%         \label{light_ep6}
%         }
%     }
%     \subfigure[Light Ep7]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/light_7.png}
%         \label{light_ep7}
%         }
%     }
%     \caption{Showing the Confidence intervals for MAP Upper Bounds for different epochs for GCN model on Cora Graph Dataset with light noise.}
% \end{figure*}

% \begin{figure*}

%     \centering
%     \subfigure[Extreme Ep0]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/extreme_0.png}
%         \label{extreme_ep0}
%         }
%     }
%     \subfigure[Extreme Ep1]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/extreme_1.png}
%         \label{extreme_ep1}
%         }
%     }
%     \subfigure[Extreme Ep2]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/extreme_2.png}
%         \label{extreme_ep2}
%         }
%     }
%     \subfigure[Extreme Ep3]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/extreme_3.png}
%         \label{extreme_ep3}
%         }
%     }
%     \subfigure[Extreme Ep4]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/extreme_4.png}
%         \label{extreme_ep4}
%         }
%     }
%     \subfigure[Extreme Ep5]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/extreme_5.png}
%         \label{extreme_ep5}
%         }
%     }
%     \subfigure[Extreme Ep6]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/extreme_6.png}
%         \label{extreme_ep6}
%         }
%     }
%     \subfigure[Extreme Ep7]{\scalebox{0.4}{
%         \includegraphics{figs/cora/gcn/extreme_7.png}
%         \label{extreme_ep7}
%         }
%     }
%     \caption{Showing the Confidence intervals for MAP Upper Bounds for different epochs for GCN model on Cora Graph Dataset with extreme noise.}
% \end{figure*}



==> old-notes.tex <==

\eat{

\section{Summary of our approach}

Almost all forms of data can be represented in the form of a graph. Unlike images or text, graphs do not have a notion of ordering and therefore, well-known methods like CNNs and RNNs do not work. Node embeddings are an integral part of machine learning in Graphs. Node embeddings are the vector representations for nodes in the graph. They should capture the graph topology, the relationship structure between nodes, and other relevant information. The notion of similarity is very widely used for embeddings. The similarity between embeddings of two entities signifies a degree of similarity in their properties. In the case of node embeddings, it could mean the nodes are similar in the graph network in some sense. This remains highly speculative and this topic has not been studied in depth and the node embeddings could carry different meanings based on the way they are trained. Therefore, in this work, we are attempting to verify the knowledge encoded by the node embeddings. Specifically, we are currently working on the Cora Citation Graph, where we look at the task of Node Classification. We obtain the node embeddings using Graph Convolution Network (GCN) trained on node classification.

We then use the \textit{homophily} property to make an assumption i.e., if two nodes are neighbors, they should share many properties and their vector representations need to be similar. \textit{Homophily} is an important concept, and an organizing principle for many real-world networks like social networks, citation networks, etc.

\section{Hybrid Markov Logic Networks}

Hybrid Markov Logic Networks (HMLNs) \cite{wang2008hmln} is a type of probabilistic graphical model that combines first-order logic and Markov random fields. HMLNs are used to represent uncertain knowledge in domains that involve both continuous and discrete variables. HMLNs represent complex systems where some variables are continuous (like temperature or pressure) and others are discrete (like on/off or true/false). HMLNs use logic to represent relationships between variables and probabilities to represent uncertainty. The "hybrid" aspect of HMLNs refers to the fact that they can represent both continuous and discrete variables. For example, an HMLN could represent a system where the temperature of a room (a continuous variable) affects whether the heating system is on or off (a discrete variable).
The "Markov" aspect of HMLNs refers to the fact that they use Markov random fields to represent the probability distribution over the variables. Markov random fields are a type of probabilistic graphical model that represents the joint probability distribution over a set of variables. The "logic" aspect of HMLNs refers to the fact that they use first-order logic to represent relationships between variables. 

HMLNs are a powerful tool for representing uncertain knowledge in complex systems that involve both continuous and discrete variables. They are used in a variety of applications, including robotics, natural language processing, and computer vision.


\subsection{Citation Network and FOL formulation}
The citation network represents articles as nodes, words in articles as node features, article topics as node labels, and citation relation as a link between nodes.

Neighbors(A, B) represents nodes A and B have a link.

Class(A, c1) represents the class label of node A is c1.

SameClass(A, B) represents nodes A and B have the same class label.

Dist(A, B) represents the distance between nodes A and B in the embedding space.

Dist(A, B) < k represents the soft inequality.

\subsubsection{FOL Formulas}
$
Neighbors(A,B) \land Class(A, cls) \Longrightarrow Class(B, cls)\\
Dist(A,B) < k * [Class(A, cls) \Longleftrightarrow Class(B, cls)]\\
Class(A, cls) \land Class(B, cls) \Longleftrightarrow SameClass(A, B)
$

\section{Mixture Models}
Learning a mixture model for the different threshold value of distance.

\section{Experiments Plan}

First, formulate the problem of HMLN inference as an Integer Linear Programming problem. Each first-order logic formula can be expressed as a set of constraints.
Ground the formulas and derive the constraints to add to the ILP solver.

A first order logic formula can be thought of as a constraint which limits or guides the truth value assignment of ground atoms. We convert a FOL formula into its Conjunctive Normal Form (CNF) and each of the disjunctions can be represented by a linear equation. For example: 

$
[Class(A, cls) \Longleftrightarrow Class(B, cls)] \Longleftrightarrow K
$
\\
can be represented in CNF as:\\
$
(Class(A, cls) \lor \neg Class(B, cls) \lor \neg K ) \land 
(\neg Class(A, cls) \lor Class(B, cls) \lor \neg K ) \land 
(\neg Class(A, cls) \lor \neg Class(B, cls) \lor K ) \land 
(Class(A, cls) \lor Class(B, cls) \lor K )
$

Each of the disjunctions can now be converted into a linear equation. For example, $Class(A, cls) \lor \neg Class(B, cls) \lor \neg K$ can be rewritten as:

$
Class(A,cls) + (1 - Class(B,cls)) + (1 - K) > 0\\
Class(B,cls) + K - Class(A,cls) \leq 1
$

And thus, every FOL formula can be represented as a set of linear equations. These linear equations resemble the constraints for an ILP optimization problem. In order to encode the MAP task as ILP optimization in Gurobi, we do the following:

\item Form the FOL formulas describing the relations in the data.
\item 

Add the concept of weight-sharing among different groundings of a formula.



\section{Lit Review}
Similar/Follow-up works on HMLNs. \cite{MLN_Num_Constr, DBLP:journals/corr/BachBHG15, info12030124, dominik2010}

Related work on Mixed Integer Linear Programming: \cite{DBLP:journals/corr/abs-1205-2644}

Prior works on Embedding model evaluation. \cite{wang_wang_chen_wang_kuo_2019}

MC-SAT for MLNs. \cite{poon2006}

Importance weights for Formula on specific evidence \cite{khan2020finegrained}

Reliable Post-Hoc explanations \cite{reliable:neurips21}

Stacked Mixture Models \cite{NIPS1997_ee8374ec}

\section{Hypercube representation}

\begin{definition}
A hypercube is a vector $[S_1 \ldots S_k]$ where each $S_i$ is a set of literals. 
\end{definition}

\begin{definition}
Given two hypercubes $H_1$, $H_2$, the join operator $H_1$ $*$ $H_2$ generates a hypercube that contains all sets in $H_1$ that have no literals in common with any set in $H_2$, all sets in $H_2$ that have no literals in common with any set in $H_2$ and for two sets $S$ $\in$ $H_1$, $S'$ in $H_2$ where $S\cap S'\not = \emptyset$, $H_1*H_2$ contains $S\cap S'$.
%generates a hypercube $[Z_1 \ldots Z_m]$, where $X_i$ $\in$ $H$ if $X_i$ $\cap$ $Y_j$ $=$ $\emptyset$, $\forall j$, $Y_i$ $\in$ $H$ if $X_i$ $\cap$ $Y_j$ $=$ $\emptyset$, $\forall j$ and $X_i$ $\cap$ $Y_j$
\end{definition}

\begin{definition}
A conjunctive query (CQ) is represented by a function $\phi(x_1,\ldots x_k)$, where each $x_i$ is a variable in the query. The same function can represent several CQs.
\end{definition}

\begin{definition}
The CQ function for a hypercube $H$ $=$ $[S_1 \ldots S_k]$ is  $\phi(x_1,\ldots x_k)$, where the domain of $x_i$ is the set of literals in $S_i$.
\end{definition}

\begin{definition}
Given a CQ $C$ with CQ function $\phi(x_1,\ldots x_k)$, the induced query graph is a graph with $k$ nodes and there exists an edge between nodes $x_i$, $x_j$ if $C$ contains an atom that relates $x_i$ and $x_j$.
\end{definition}

Learning CQ-functions

Assume a prior structural constraint


\begin{definition}
The width of a hypercube $H$ is the maximum treewidth for any query graph derived from $H$.
\end{definition}



We learn a hypercube representation for the data such that its treewidth is bounded by $\epsilon$. We then train the model by a projection

Training

Each hypercube represents a query. We train the model to predict the probability of that query.


Starting off, for any data, we treat each individual data instance (data row) as nodes. We iteratively merge the nodes to get the supernodes of the hypercube. The hypercube represents a query.

\begin{definition}
    Given a pre-trained graph neural network, we want to evaluate what it has learnt with regards to the lower level relationship structure in the graph. 
\end{definition}

For this, we create query graphs of tree-width \textit{t}, which are the sub-structures from the full graph. We mask a node in the query graph and ask the pre-trained model to predict the masked node based on the neighborhoods provided in the query graph.

Query graphs of different tree-widths represent queries of different structure. As the tree-width \textit{t} increases, so does the complexity of the queries. A query graph with $\textit{t}=1$ can be thought of as a first order query. For example $\exists y: R(x, y) \wedge R(y,z)$ is a simple first order query that can be represented by a query graph of $\textit{t}=1$. It is important to note that $\textit{t}=1$ can represent sever other queries like $\exists y: R(x, y) \wedge R(y,z) \wedge R(y,a) \wedge R(y,b)$, where $a, b, y$ and $z$ are the neighbors of $y$. The number of neighbors provided can be thought of as the hints provided for the model to help predict the class label of node $y$. The intuition behind this is that if the model has actually learnt about the masked node, it should be able to predict its label correctly regardless of the neighborhood provided. The hidden vector embeddings learnt by the graph neural network for each node should already contain the information about the neighborhoods.
}

==> prelim.tex <==

\section{Background}

\subsection{First-order Logic.} The language of first-order logic (cf. \cite{genesereth&kao13}) consists of quantifiers ($\forall$ and $\exists$), logical variables, constants, predicates, and logical connectives ($\vee$, $\wedge$, $\neg$, $\Rightarrow$, and $\Leftrightarrow$). 
%We denote logical variables by lower case letters (e.g., $x$, $y$, $z$) and constants, which model objects in the real-world domain,  by strings that begin with an uppercase letter (e.g., $A$, $Ana$, $Bob$). A predicate is a relation that takes a specific number of arguments as input and outputs either {\sc true} (synonymous with $1$) or {\sc false} (synonymous with $0$). The arity of a predicate is the number of its arguments. We assume that each logical variable $x$ has a finite domain of objects $\Delta_x$ that it can be substituted with (Herbrand semantics). A ground atom is a predicate where all its variables have been substituted by a constant (we use the terms constants and objects interchangeably) from its domain. For example, ${\tt Friends}(Alice, Bob)$ is a ground atom obtained by substituting the variables in ${\tt Friends}(x,y)$.
A predicate is a relation that takes a specific number of arguments as input and outputs either {\sc true} (synonymous with $1$) or {\sc false} (synonymous with $0$). A ground atom is a predicate where all its variables have been substituted by a constant (we use the terms constants and objects interchangeably) from its domain. For example, ${\tt Friends}(Alice, Bob)$ is a ground atom obtained by substituting the variables in ${\tt Friends}(x,y)$.
A first-order formula connects predicates using logical connectives. For example, ${\tt Friends}(x,y)$ $\Rightarrow$ ${\tt Friends}(y,x)$. A grounding of a first order formula is one where all variables in the formula have been substituted by constants. For example, ${\tt Friends}(Alice,Bob)$ $\Rightarrow$ ${\tt Friends}(Bob,Alice)$. Note that a ground formula evaluates to either True or False. 

%A knowledge-base is a set of first-order formulas.

%A term is either a logical variable or a constant. We denote predicates by strings in typewriter font  (e.g., $\texttt{R}$, $\texttt{Smokes}$) followed by a parenthesized list of terms. 

%A first-order formula is recursively defined as follows:\begin{inparaenum}[(i)]\item An atomic formula (atom) is a predicate; \item Negation of an atom is a formula; \item If $f$ and $g$ are formulas then connecting them by binary connectives such as $\wedge$ and $\vee$ yields a formula; and \item If $f$ is a formula and $x$ is a logical variable then $\forall x f$ and $\exists x f$ are formulas\end{inparaenum}. A first-order knowledge base (KB) is a set of first-order formulas. 

%We assume that each argument of each predicate is typed and can only be assigned to a finite set of constants. By extension, each logical variable in each formula is also typed. 

%We assume that our language does not contain the equality symbol and function symbols. We further assume that all first-order formulas are disjunctive (clauses), have no free logical variables, have only universally quantified logical variables (namely, the KB is in conjunctive normal form (CNF)), and have no constants. Note that all first-order formulas can be easily converted to this form. 

%A ground atom is an atom that contains no logical variables. A ground formula is a formula containing only ground atoms. The grounding of a first-order formula $f$ is the set of all possible ground formulas that can be obtained from $f$ by substituting all the logical variables in it by constants in their domain. A ground KB is obtained from a first-order KB by grounding all of its first-order formulas. A possible world, denoted by $\omega$, is a truth assignment to all possible ground atoms in the first-order KB. 

\subsection{Markov Logic Networks} 

%Markov logic networks (MLNs) are symbolic models that represent uncertain domain knowledge using the language of first-order logic and probabilistic graphical models. Specifically, a formula in an MLN represents relational dependencies across different variables in the model. Each formula in an MLN has a real-valued weight which is shared across all instantiations of the formula (called groundings of the formula). Weights are typically learned by maximizing the likelihood of a relational database~\cite{domingos&lowd09} Learning an MLN is computationally hard since computing the gradient requires inference over a large probabilistic graphical model. The MLN with learned weights represents a Markov network, where each ground formula is a potential in the Markov network. 

Markov logic networks (MLNs) soften the satisfiability constraint in first-order logic using weights attached to each first-order formula. Each formula in an MLN has a real-valued weight which is shared across all groundings of that formula. For example, ${\tt Friends}(x,y)$ $\Rightarrow$ ${\tt Friends}(y,x)$; $w$, where $w$ is the weight. Weights are typically learned by maximizing a likelihood function of an observed world~\cite{domingos&lowd09}. The MLN represents a probability distribution (a Markov network) over possible worlds, where a world is an assignment (of either 1 or 0) to every ground atom in the MLN. 
\eat{
The distribution is given by,

 \begin{equation}
 \Pr(\omega) = \frac{1}{Z} \exp \left ( \sum_{i} w_i N_{i}(\omega) \right ) \label{eq:mln_prob_dist}
\end{equation}  
where $w_i$ is the weight of formula $f_i$, $N_{i}({\omega})$ is the number of groundings of formula $f_i$ that evaluate to True given a world
$\omega$, and $Z$ is the normalization constant.
}
%The first-order structure in the formula means that the dependencies hold for all instantiations of a formula

%Markov logic networks (MLNs) are template models that define uncertain, relational knowledge as first-order formulas with weights. Weights encode uncertainty in a formula. $\infty$ weight formulas are hard constraints which should always be true. Similarly formulas with $-\infty$ weights are always false. Thus, MLNs offer a flexible framework to mix hard and soft formulas. In MLNs, we assume that each argument of each predicate in the MLN is typed and can only be assigned to a finite set of constants. By extension, each logical variable in each formula is also typed. Thus, each variable corresponds to a specific domain of objects. A ground atom is an atom where each of its variables have been substituted by constants from their respective domains. A ground formula is a formula containing only ground atoms.
\eat{
Given a set of constants that represent the domains of variables in the MLN, an MLN represents a factored probability distribution over the possible worlds, in the form of a Markov network. A world in an MLN is an assignment of 0/1 to all ground atoms of the MLN. Specifically, the distribution is given by,
 \begin{align} \Pr(\omega) &
= \frac{1}{Z} \exp \left ( \sum_{i} w_i N_{i}(\omega) \right ) \label{eq:mln_prob_dist}
\end{align} where $w_i$ is the weight of formula $f_i$, $N_{i}({\omega})$ is the number of groundings of formula $f_i$ that evaluate to True given a world
$\omega$, and $Z$ is the normalization constant.
}
The two common inference problems over MLNs are (1) given observed evidence, compute the marginal probability distribution of a ground atom in the ground Markov network (2) given observed evidence, perform MAP inference where we compute the most probable assignment to all non-evidence atoms. Both queries are computationally hard, and therefore require approximate inference methods.
\eat{
Important inference queries in MLNs are computing the partition function, finding the
marginal probability of an atom given evidence (an assignment to a subset of variables) and finding
the most probable assignment to all atoms given evidence (MAP inference). Here, we focus on the marginal inference problem.
}

%As a simple example of an MLN, suppose we want to encode the fact that smokers and asthmatics are not friends. We would design an MLN with a formula such as $\texttt{Smokes}(x)$ $\wedge$ $\texttt{Friends}(x,y)$ $\Rightarrow$ $\neg Asthma(y)$. Given constants corresponding to the variables, $x$ and $y$, the MLN represents a joint distribution over all ground atoms of $\texttt{Smokes}$, $\texttt{Friends}$, and $\texttt{Asthma}$. 


%The two key tasks in MLNs are {\em weight learning}, which is the task of learning  the weights attached to the formulas from a relational database, and {\em inference} (prediction),
%which is the task of answering queries posed over the learned model given observations (evidence database). In marginal inference, we compute the probability of a query given evidence, while in MAP we maximize the joint probability of the non-evidence variables.
%The two main inference problems over MLNs are (1) posterior or marginal estimation which involves finding the marginal probability distribution of a random variable (ground atom) in the ground Markov network given an evidence database. For example computing the probability that $\texttt{Smokes}(Ana)$ is true given $\texttt{Smokes}(Bob)$ is true and $\texttt{Friends}(Ana, Bob)$ is true. (2) Maximum-a-posteriori (MAP) estimation which involves finding an assignment of values to all non-evidence variables such that the assignment has the maximum probability. For example, given that $\texttt{Smokes}(Ana)$, $\texttt{Smokes}(Bob)$ and $\texttt{Friends}(Ana, Bob)$ is true, what is the assignment to all other ground atoms in the MLN such that their joint probability is maximum.


%Both marginal inference and MAP inference are \#P-hard and NP-hard in general respectively. Several interesting tasks such as structured prediction and joint inference are special cases of these inference tasks. 
%Weights attached to first-order formulas can be learned either {\em generatively}, in which the goal is to find weights that maximize the log-likelihood of the data, or {\em discriminatively}, in which the goal is to maximize the conditional log-likelihood of the data given evidence. In principle, both tasks can be solved using a standard gradient ascent procedure with appropriate regularization constraints. However, it turns out that computing the gradient is computationally intractable, since the problem of computing the gradient can be reduced to the posterior marginal estimation task. Therefore, practitioners often use alternate objective criteria such as contrastive divergence \cite{hinton02}, voted perceptron \cite{collins02}, and pseudo log-likelihood \cite{besag75} since the gradient of these functions is easier to compute.

\input{related}
